QCluster: Clustering Packets for Flow Scheduling

Flow scheduling is crucial in data centers, as it directly influences user experience of applications. According to different assumptions and design goals, there are four typical flow scheduling problems/solutions: SRPT, LAS, Fair Queueing, and Deadline-Aware scheduling. When implementing these solutions in commodity switches with limited number of queues, they need to set static parameters by measuring traffic in advance, while optimal parameters vary across time and space. This paper proposes a generic framework, namely QCluster, to adapt all scheduling problems for limited number of queues. The key idea of QCluster is to cluster packets with similar weights/properties into the same queue. QCluster is implemented in Tofino switches, and can cluster packets at a speed of 3.2 Tbps. To the best of our knowledge, QCluster is the fastest clustering algorithm. Experimental results in testbed with programmable switches and ns-2 show that QCluster reduces the average flow completion time (FCT) for short flows up to 56.6%, and reduces the overall average FCT up to 21.7% over state-of-the-art. All the source code in ns-2 is available in Github without.

==> acknowledgement.tex <==
\presec
\section*{Acknowledgment} 
\postsec

This work is supported by Key-Area Research and Development Program of Guangdong Province 2020B0101390001, National Natural Science Foundation of China (NSFC) (No. U20A20179, 61832001).

==> figure/2020Testbed/Alpha/alpha_vary.tex <==
\begin{figure*}[!htbp]
\centering
\subfigure[QC-FQ-1]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/2020Testbed/Alpha/Alpha1-crop.pdf}
\postsubfig
\label{fig:tb_alpha:vary:1}
\end{minipage}
}
\subfigure[QC-FQ-2]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/2020Testbed/Alpha/Alpha2-crop.pdf}
\postsubfig
\label{fig:tb_alpha:vary:2}
\end{minipage}
}
\subfigure[QC-FQ-3]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/2020Testbed/Alpha/Alpha3-crop.pdf}
\postsubfig
\label{fig:tb_alpha:vary:3}
\end{minipage}
}
\subfigure[QC-FQ-4]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/2020Testbed/Alpha/Alpha4-crop.pdf}
\postsubfig
\label{fig:tb_alpha:vary:4}
\end{minipage}
}
\postsubfig
\caption{Change of alpha over time for QC-FQ on W6 in testbed. Finally alpha parameters for each two queues will converge into very close values respectively.}
\label{fig:tb_alpha:vary}
\end{figure*}

==> figure/2020Testbed/Dist/dist_vary_Rem.tex <==
\begin{figure}[!h]
\centering
\subfigure[QC-FQ-2]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/2020Testbed/Dist/Dist2-crop.pdf}
\postsubfig
\label{fig:tb_dist:vary:3}
\end{minipage}
}
\subfigure[QC-FQ-4]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/2020Testbed/Dist/Dist4-crop.pdf}
\postsubfig
\label{fig:tb_dist:vary:4}
\end{minipage}
}
\postsubfig
\caption{Change of packet distributions over time for QC-FQ on W6 in testbed. The packet distribution is the proportion of packets in one queue among all packets.}
\label{fig:tb_dist_Rem:vary}
\end{figure}

==> figure/2020Testbed/Thres/thres_vary_Rem.tex <==
\begin{figure}[!h]
\centering
\subfigure[QC-FQ-2]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/2020Testbed/Thres/Thres2-crop.pdf}
\postsubfig
\label{fig:tb_thres:vary:3}
\end{minipage}
}
\subfigure[QC-FQ-4]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/2020Testbed/Thres/Thres4-crop.pdf}
\postsubfig
\label{fig:tb_thres:vary:4}
\end{minipage}
}
\postsubfig
\caption{Change of thresholds over time for QC-FQ on W6 in testbed.}
\label{fig:tb_thres_Rem:vary}
\end{figure}

==> figure/FCT/W5.tex <==
\begin{figure*}[!htbp]
%\centering
\subfigure[(0,1KB): Avg]{
\begin{minipage}[b]{0.235\textwidth}
\centering
\includegraphics[width=1.09\textwidth]{figure/FCT/W5_1K.pdf}
\end{minipage}
}
\subfigure[(0,1KB): 99th Percentile]{
\begin{minipage}[b]{0.235\textwidth}
\centering
\includegraphics[width=1.09\textwidth]{figure/FCT/W5_99th.pdf}
\end{minipage}
}
\subfigure[(1KB,10KB): Avg]{
\begin{minipage}[b]{0.235\textwidth}
\centering
\includegraphics[width=1.09\textwidth]{figure/FCT/W5_10K.pdf}
\end{minipage}
}
\subfigure[(10KB,$\infty$): Avg]{
\begin{minipage}[b]{0.235\textwidth}
\centering
\includegraphics[width=1.09\textwidth]{figure/FCT/W5_10K+.pdf}
\end{minipage}
}
\caption{W5: FCT across different flow sizes.}
\label{fig:W5}
\end{figure*}

==> figure/FCT_AVG/AVG_Rem.tex <==
\begin{figure*}[!htbp]
\centering
\subfigure[W1]{
\begin{minipage}[b]{0.235\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{sigcomm20/figure/former/W1-crop.pdf}
\postsubfig
\label{fig:AVG:W1}
\end{minipage}
}
\subfigure[W2]{
\begin{minipage}[b]{0.24\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{sigcomm20/figure/former/W2-crop.pdf}
\postsubfig
\label{fig:AVG:W2}
\end{minipage}
}
\subfigure[W3]{
\begin{minipage}[b]{0.24\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{sigcomm20/figure/former/W3-crop.pdf}
\postsubfig
\label{fig:AVG:W3}
\end{minipage}
}
\subfigure[W5]{
\begin{minipage}[b]{0.225\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{sigcomm20/figure/former/W5-crop.pdf}
\postsubfig
\label{fig:AVG:W5}
\end{minipage}
}
\postsubfig
\caption{Overall average FCT on the remaining four workloads for SRPT and LAS.}
\label{fig:AVG_Rem}
\end{figure*}

==> figure/FCTall/all.tex <==
\begin{figure*}[!htbp]
%\centering
\subfigure[(0, 1KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/keyvalue_1K-cropped.pdf}
\end{minipage}
}
\subfigure[(0, 1KB): 99th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/keyvalue_99th-cropped.pdf}
\end{minipage}
}
\subfigure[(1KB,10KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/keyvalue_10K-cropped.pdf}
\end{minipage}
}
\subfigure[(10KB,$\infty$): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/keyvalue_10K+-cropped-1.pdf}
\end{minipage}
}
\caption{W1: FCT across different flow sizes.}
\label{fig:keyvalue}
\end{figure*}

\begin{figure*}[!htbp]
%\centering
\subfigure[(0, 1KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/allrpc_1K-cropped.pdf}
\end{minipage}
}
\subfigure[(0, 1KB): 99th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/allrpc_99th-cropped.pdf}
\end{minipage}
}
\subfigure[(1KB,10KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/allrpc_10K-cropped.pdf}
\end{minipage}
}
\subfigure[(10KB,$\infty$): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/allrpc_10K+-cropped-1.pdf}
\end{minipage}
}
\caption{W3: FCT across different flow sizes.}
\label{fig:allrpc}
\end{figure*}

\begin{figure*}[!htbp]
%\centering
\subfigure[(0, 1KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/vl2_1K-cropped.pdf}
\end{minipage}
}
\subfigure[(0, 1KB): 99th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/vl2_99th-cropped.pdf}
\end{minipage}
}
\subfigure[(1KB,10KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/vl2_10K-cropped.pdf}
\end{minipage}
}
\subfigure[(10KB,$\infty$): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/vl2_10K+-cropped-1.pdf}
\end{minipage}
}
\caption{W5: FCT across different flow sizes.}
\label{fig:vl2}
\end{figure*}

\begin{figure*}[!htbp]
\subfigure[(0KB, 10KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/search_1K-cropped.pdf}
\end{minipage}
}
\subfigure[(0, 10KB): 99th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/search_99th-cropped.pdf}
\end{minipage}
}
\subfigure[(10KB,100KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/search_10K-cropped.pdf}
\end{minipage}
}
\subfigure[(100KB,$\infty$): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/search_10K+-cropped-1.pdf}
\end{minipage}
}
\caption{W6: FCT across different flow sizes.}
\label{fig:search}
\end{figure*}



==> figure/FCTall/appendfigure.tex <==
\begin{figure*}[!htbp]
%\centering
\subfigure[(0, 1KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/keyvalue_1K-cropped.pdf}
\end{minipage}
}
\subfigure[(0, 1KB): 99th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/keyvalue_99th-cropped.pdf}
\end{minipage}
}
\subfigure[(1KB,10KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/keyvalue_10K-cropped.pdf}
\end{minipage}
}
\subfigure[(10KB,$\infty$): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/keyvalue_10K+-cropped-1.pdf}
\end{minipage}
}
\caption{W1: FCT across different flow sizes.}
\label{fig:keyvalue}
\end{figure*}

\begin{figure*}[!htbp]
%\centering
\subfigure[(0, 1KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/allrpc_1K-cropped.pdf}
\end{minipage}
}
\subfigure[(0, 1KB): 99th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/allrpc_99th-cropped.pdf}
\end{minipage}
}
\subfigure[(1KB,10KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/allrpc_10K-cropped.pdf}
\end{minipage}
}
\subfigure[(10KB,$\infty$): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/allrpc_10K+-cropped-1.pdf}
\end{minipage}
}
\caption{W3: FCT across different flow sizes.}
\label{fig:allrpc}
\end{figure*}

\begin{figure*}[!htbp]
%\centering
\subfigure[(0, 1KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/vl2_1K-cropped.pdf}
\end{minipage}
}
\subfigure[(0, 1KB): 99th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/vl2_99th-cropped.pdf}
\end{minipage}
}
\subfigure[(1KB,10KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/vl2_10K-cropped.pdf}
\end{minipage}
}
\subfigure[(10KB,$\infty$): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/vl2_10K+-cropped-1.pdf}
\end{minipage}
}
\caption{W5: FCT across different flow sizes.}
\label{fig:vl2}
\end{figure*}

\begin{figure*}[!htbp]
\subfigure[(0KB, 10KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/search_1K-cropped.pdf}
\end{minipage}
}
\subfigure[(0, 10KB): 99th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/search_99th-cropped.pdf}
\end{minipage}
}
\subfigure[(10KB,100KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/search_10K-cropped.pdf}
\end{minipage}
}
\subfigure[(100KB,$\infty$): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/FCTall/search_10K+-cropped-1.pdf}
\end{minipage}
}
\caption{W6: FCT across different flow sizes.}
\label{fig:search}
\end{figure*}

==> figure/FCTddl/fctddl.tex <==
\begin{figure}[h!]
%\centering
\subfigure[100K]{
\begin{minipage}[b]{0.23\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/FCTddl/100K-cropped.pdf}
\end{minipage}
}
\subfigure[Average FCT]{
\begin{minipage}[b]{0.215\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/FCTddl/all-cropped.pdf}
\end{minipage}
}
\presec
\presec
\caption{FCTddl}
\label{fig:FCTddl}
\end{figure}

==> figure/Mem/Mem.tex <==
\begin{figure*}[!htbp]
\subfigure[(0KB, 10KB): Avg]{
\begin{minipage}[b]{0.248\textwidth}
\centering
\includegraphics[width=\textwidth]{sigcomm20/figure/Mem/Mem1-crop.pdf}
\postsubfig
\label{fig:Mem:10K}
\end{minipage}
}
\subfigure[(0, 10KB): 95th Percentile]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{sigcomm20/figure/Mem/Mem2-crop.pdf}
\postsubfig
\label{fig:Mem:95th}
\end{minipage}
}
\subfigure[(10KB,100KB): Avg]{
\begin{minipage}[b]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{sigcomm20/figure/Mem/Mem3-crop.pdf}
\postsubfig
\label{fig:Mem:100K}
\end{minipage}
}
\subfigure[(100KB,$\infty$): Avg]{
\begin{minipage}[b]{0.22\textwidth}
\centering
\includegraphics[width=\textwidth]{sigcomm20/figure/Mem/Mem4-crop.pdf}
\postsubfig
\label{fig:Mem:infty}
\end{minipage}
}
\postsubfig
\caption{FCT across different flow sizes on W6 for QC-LAS using \# buckets SCM sketch.}
\label{fig:Mem}
\end{figure*}

==> figure/Memory/Memory.tex <==
\begin{figure}[h!]
%\centering
\subfigure[(0,100KB): Avg]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/Memory/W6_10K.pdf}
\end{minipage}
}
\subfigure[Overall: Avg]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/Memory/W6_AVG.pdf}
\end{minipage}
}
\caption{W6: FCT comparisons under different memory usage.}
\label{fig:Memory}
\end{figure}

==> figure/Memory_old/Memory.tex <==
\begin{figure}[h!]
%\centering
\subfigure[(0,100KB): Avg]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/Memory/W6_10K_div.pdf}
\end{minipage}
}
\subfigure[Overall: Avg]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/Memory/W6_AVG_div.pdf}
\end{minipage}
}
\caption{W6: FCT comparisons under different memory usage.}
\label{fig:Memory}
\end{figure}

==> figure/PDA/PDA_FCT.tex <==
\begin{figure}[h!]
%\centering
\subfigure[W4]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{sigcomm20/figure/PDA/PDA_W4-crop.pdf}  
\postsubfig
\label{fig:PDA_FCT:W4}
\end{minipage}
}
\subfigure[W6]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{sigcomm20/figure/PDA/PDA_W6-crop.pdf} 
\postsubfig
\label{fig:PDA_FCT:W6}
\end{minipage}
}
\postsubfig
\caption{\zyk{Impact of packet disorder avoidance on FCT for SRPT and LAS.}}
\label{fig:PDA_FCT}
\end{figure}
%\postsec

==> figure/PDA/PDA_POR.tex <==
\begin{figure}[h!]
%\centering
\subfigure[W4]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{sigcomm20/figure/PDA/ORDER_W4-crop.pdf}  
\postsubfig
\label{fig:PDA_POR:W4}
\end{minipage}
}
\subfigure[W6]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{sigcomm20/figure/PDA/ORDER_W6-crop.pdf} 
\postsubfig
\label{fig:PDA_POR:W6}
\end{minipage}
}
\postsubfig
\caption{\zyk{Impact of packet disorder avoidance on packet ordered ratio for SRPT and LAS.}}
\label{fig:PDA_POR}
\end{figure}
%\postsec

==> figure/PIFO/PIFO_DET.tex <==
\begin{figure}[h!]
%\centering
\subfigure[(0KB,100KB): Avg]{
\begin{minipage}[b]{0.233\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/PIFO/PIFO_1-crop.pdf}  
\postsubfig
\label{fig:PIFO_DET:Small}
\end{minipage}
}
\subfigure[(100KB,$\infty$): Avg]{
\begin{minipage}[b]{0.217\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/PIFO/PIFO_2-crop.pdf} 
\postsubfig
\label{fig:PIFO_DET:Large}
\end{minipage}
}
\postsubfig
\caption{FCT comparisons with PIFO across different flow sizes on W6 for LAS.}
\label{fig:PIFO_DET}
\end{figure}
%\postsec

==> figure/PIFO/PIFO_OVE.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.64\linewidth]{sigcomm20/figure/PIFO/PIFO_0-crop.pdf}
\vvv \vvv
\caption{\zyk{FCT comparisons with PIFO on W6 for LAS.}}
%\postsubfig
\label{fig:PIFO_OVE}
\end{figure}

==> figure/Queue/Queue.tex <==
\begin{figure}[h!]
%\centering
\subfigure[QC-SRPT]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/former/SRPT-crop.pdf}
\postsubfig
\label{fig:Queue:known}
\end{minipage}
}
\subfigure[QC-LAS]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/former/LAS-crop.pdf}
\postsubfig
\label{fig:Queue:unknown}
\end{minipage}
}
\postsubfig
\caption{FCT comparisons under different queue numbers on W4 for SRPT and LAS.}
\label{fig:Queue}
\end{figure}
%\postsec

==> figure/Queue_old/Queue.tex <==
\begin{figure}[h!]
%\centering
\subfigure[QC-SRPT]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/Queue/Known_W4_AVG.pdf}
\end{minipage}
}
\subfigure[QC-LAS]{
\begin{minipage}[b]{0.22\textwidth}
%\centering
\includegraphics[width=\textwidth]{figure/Queue/Unknown_W4_AVG.pdf}
\end{minipage}
}
\caption{W4: FCT comparisons under different queue number.}
\label{fig:Queue}
\end{figure}

==> figure/testbed/testbed_topology.tex <==
\begin{figure}[h!]
\centering
\presub
\includegraphics[width=0.35\linewidth]{figure/testbed/testbed_topology.pdf}
\includegraphics[width=0.64\linewidth]{figure/testbed/testbed-cropped.pdf}
\vvv \vvv \vvv \vspace{-0.12in}
\caption{Topology and deployment of our testbed.
}
\vvv \vvv
\label{fig:tdt}
\end{figure}
